Kernel Stein Discrepancy Descent

Among dissimilarities between probability distributions, the Kernel Stein Discrepancy (KSD) has received much interest recently. We investigate the properties of its Wasserstein gradient flow to approximate a target probability distribution $\pi$ on $\mathbb{R}^d$, known up to a normalization constant. This leads to a straightforwardly implementable, deterministic score-based method to sample from $\pi$, named KSD Descent, which uses a set of particles to approximate $\pi$. Remarkably, owing to a tractable loss function, KSD Descent can leverage robust parameter-free optimization schemes such as L-BFGS; this contrasts with other popular particle-based schemes such as the Stein Variational Gradient Descent algorithm. We study the convergence properties of KSD Descent and demonstrate its practical relevance. However, we also highlight failure cases by showing that the algorithm can get stuck in spurious local minima.

==> KSD descent/auxiliary_results.tex <==

\begin{lemma}
	Assume that $k : \R^n \times \R^n \rightarrow \R$ is a kernel, such that $k(\cdot, x)$ is $\lambda$-convex for all $x \in \R^n$. Let $H$ be the RKHS of $k$ and assume it is separable. Then the functional
	$$\mathcal{W}_k = \int_{\R^n}\int_{\R^n} k(x,y) \mu(dx) \mu(dy)$$
	is $\lambda$-geodesically convex on $(\mathcal{P}_2(\R^n), W_2)$.
\end{lemma}
\begin{proof}
	Let $\mu_0, \mu_1 \in \mathcal{P}_2(\R^n) \cap \mathcal{P}_k(\R^n)$. Since the kernel is measurable and RKHS $H$ is separable, the kernel mean embeddings:
	$$ \hat{\mu}_i = \int k(\cdot, x) \mu_i(dx) $$
	exist for $i \in \{0,1\}$. Furthermore, $\mathcal{W}_k(\mu_i) = \Vert \hat{\mu}_i \Vert_H^2$ for $i \in \{0,1\}$. 
	
	Let $\pi \in \Pi(\mu, \nu)$ be an optimal transport plan between $\mu_0$ and $\mu_1$ and let $0 < t < 1$. We have:
	\begin{align*}
	\mathcal{W}_k(\mu_t) = & \iint k((1-t) x_1 + tx_2 , (1-t) y_1 + ty_2)  \pi(dx_1, dx_2) \pi(dy_1, dy_2)  \\ 
	&\leq  \iint (1-t) k(x_1, (1-t)y_1 + t y_2) + t k(x_2, (1-t)y_1 + ty_2) - t(1-t)\frac{\lambda}{2} \Vert x_1 - x_2 \Vert_2^2 \pi(dx_1, dx_2) \pi(dy_1, dy_2)  \\
	& \leq \iint (1-t)^2 k(x_1, y_1) + t(1-t) (k(x_1, y_2) + k(x_2, y_1)) + t^2 k(x_2, y_2) \pi(dx_1, dx_2) \pi(dy_1, dy_2) \\
	& \hspace{10pt} - \iint t(1-t)\frac{\lambda}{2} (\Vert x_1 -x_2 \Vert_2^2 + \Vert y_1 - y_2 \Vert_2^2) \pi(dx_1, dx_2) \pi(dy_1, dy_2) \\
	& = \Vert (1-t) \hat{\mu}_0 +  t\hat{\mu}_1 \Vert_H^2 - t(1-t)\lambda W_2^2(\mu_0, \mu_1) \\
	& = (1-t) \mathcal{W}_k(\mu_0) + t \mathcal{W}_k(\mu_1) - t(1-t) \Vert \hat{\mu}_0 - \hat{\mu}_1 \Vert_H^2 - \lambda t(1-t) W_2^2(\mu_0, \mu_1) \\
	& \leq  (1-t) \mathcal{W}_k(\mu_0) + t \mathcal{W}_k(\mu_1) - \lambda t(1-t) W_2^2(\mu_0, \mu_1)
	\end{align*}
	which proves the thesis.
	
	
	\begin{lemma}{Distance to constant functions}
		
		Let $f: \R^p \to \R$ such that for all $x$, the mapping $y\mapsto k_{\pi}(x, y) f(y)$ is integrable and call $\phi(x) = \int_{y} k_{\pi}(x, y) f(y) dy - 1$.
		Using Fubini, we find:
		$\int_{x} \phi(x) \pi(x)dx = -1$.
		Then, for a target measure $\mu$ such that $\pi / \mu$ is defined everywhere, it holds
		\begin{align*}
		1 &= \left\lvert\int_{x} \phi(x) \pi(x)dx\right\lvert\\
		&= \left\lvert\int_{x} \phi(x) \sqrt{\mu(x)} \frac{\pi(x)}{\sqrt{\mu(x)}}dx\right\lvert\\
		&\leq \left(\int_x \phi^2(x)d\mu(x)\right)\times \left(\int_{x}\frac{d\pi}{d\mu}(x) d\pi(x)\right)
		\end{align*}
		Which gives the bound
		$$
		\|\phi\|_{L^2(\mu)} \geq \left(\int_{x}\frac{d\pi}{d\mu}(x) d\pi(x)\right)^{-1}
		$$
	\end{lemma}
\end{proof}

\begin{lemma}{Analysis of stationary points}
	
	Consider a $2$d case, and a density $\pi$ symmetric w.r.t. the $y$ axis, i.e. $\pi(x, y) = \pi(-x, y)$. We call $\mathcal{M}$ the axis.
	
	We call $\tilde{\pi}$ the density $\R \to \R$ such that $\tilde{\pi}(0, y) \propto \pi(0, x)$.
	%
	
	Let $\mu : \R^2\to \R$ a density such that $\supp(\mu)\subset \mathcal{M}$.
	%
	We call $\tilde{\mu}$ the projection of $\mu$ on $\mathcal{M}$.
	We assume that $k$ is written as $k(x, y) = \phi(\|x - y\|^2)$, with $\phi$ decreasing.
	
	We find:
	
	$$
	KSD^2(\mu, \pi) = KSD^2(\tilde{\mu},\tilde{\pi}) - \int_{\mathcal{M}^2} \phi'(\|x -y\|)^2 d\tilde{\mu}(x)d\tilde{\mu}(y)
	$$
	
	Let $\tilde{\mu} = (I + \psi)_{\#}\tilde{\pi}$.
	%
	A Taylor development gives:
	
	$$
	KSD^2(\mu, \pi) =-\int_{\mathcal{M}^2} \phi'(\|x -y\|)^2 d\tilde{\pi}(x)d\tilde{\pi}(y) 
	-\int_{\mathcal{M}^2} \phi"(\|x -y\|)^2\langle x - y, \psi(x) - \psi(y)\rangle d\tilde{\pi}(x)d\tilde{\pi}(y)  
	+\frac12\mathrm{Hess}_{\tilde{\pi}}(\psi, \psi)
	$$
\end{lemma}


==> KSD descent/background.tex <==
\section{Background}\label{sec:background}

This section introduces the high-level idea of the gradient flow approach to sampling. It also summarizes the known properties of the KSD.

\subsection{Notations}\label{sec:notations}

The space of $l$ continuously differentiable functions on $\X$ is $C^{l}(\X)$. The space of smooth functions with compact support is $C_c^{\infty}(\X)$. 
If $\psi : \X \to \R^p$ is differentiable, we denote by $J \psi : \X \to \R^{p \times d}$ its Jacobian. %If $p = 1$, the gradient of $\psi$ denoted $\nabla \psi$ is seen as a column vector.
If $p = 1$, we denote by $\nabla \psi$ the gradient of $\psi$.
Moreover, if $\nabla \psi$ is differentiable, the Jacobian of $\nabla \psi$ is the Hessian of $\psi$ denoted $H \psi$. If $p = d$, $\div \psi$ denotes the divergence of $\psi$, i.e.\ the trace of the Jacobian. We also denote by $\Delta \psi$ the Laplacian of $\psi$, where $\Delta \psi=\div\nabla \psi$. 
For a differentiable kernel $k: \R^{d} \times \R^{d} \rightarrow \R,$ $\nabla_{1} k$ (resp. $\nabla_{2} k$) is the gradient of the kernel w.r.t. the first (resp. second) variable, while $H_1 k$ denotes its Hessian w.r.t.\ the first variable.%: \R^{d} \times \R^{d} \rightarrow \R^{d}
 
 Consider the set $\cP_2(\X)$ of probability measures $\mu$ on $\X$ with finite second moment and  $\cP_c\left(\X\right)$ the set of probability measures with compact support. For $\mu \in \cP_2(\X)$, we denote by $\d\mu/\d\pi$ its Radon-Nikodym density if $\mu$ is absolutely continuous w.r.t.\ $\pi$.  For any $\mu \in \cP_2(\X)$, $L^2(\mu)$ is the space of functions $f : \X \to \R$ such that $\int \|f\|^2 d\mu < \infty$. %Note that the identity map $I$ is an element of $L^2(\mu)$. 
 We denote by $\Vert \cdot \Vert_{L^2(\mu)}$ and $\ps{\cdot,\cdot}_{L^2(\mu)}$ respectively the norm and the inner product of the Hilbert space $L^2(\mu)$. 
Given a measurable map $T:\X\to \X$ and $\mu\in \cP_2(\X)$, $T_{\#}\mu$ is the pushforward measure of $\mu$ by $T$. %, characterized by the transfer lemma for any measurable and bounded function $\phi$: $\int \phi(T(x))d\mu(x)=\int \phi(y)dT_{\#}\mu(y)$.
We consider, for $\mu,\nu \in \cP_2(\X)$, the 2-Wasserstein distance $W_2 (\mu, \nu)$, %, i.e.\ the set of nonnegative measures $s$ over $\X \times \X$ such that $P_{\#} s = \mu$ (resp. $Q_{\#} s = \nu$) where $P : (x,y) \mapsto x$ (resp. $Q : (x,y) \mapsto y$) denotes the projection onto the first (resp. the second) component.   = \inf_{s \in \mathcal{S}(\mu,\nu)} \int \|x-y\|^2 ds(x,y)$, where $\mathcal{S}(\mu,\nu)$ is the set of couplings between $\mu$ and $\nu$ It is a distance over $\cP_2(\X)$, 
and we refer to the metric space $(\cP_2(\X),W_2)$ as the Wasserstein space. In a Riemannian interpretation of $(\cP_2(\X),W_2)$, the tangent space of $\cP_2(\X)$ at $\mu$ is denoted $\mathcal{T}_{\mu}\cP_2(\X)$ and is a subset of $L^2(\mu)$ \cite{otto2001geometry}. We refer to \Cref{sec:W2_diff} for more details on the Wasserstein distance and related flows.

%\subsection{Continuity equation}

\subsection{Lyapunov analysis and gradient flows}
\label{sec:sub_Lyap}

To sample from a target distribution $\pi$, a now classical approach consists in identifying a continuous process which moves particles from an initial probability distribution $\mu_0$ toward samples of $\pi$. This can be expressed as searching for vector fields $v_t:\R^d\rightarrow \R^d$ transporting the distribution $\mu_t$ through the continuity equation (see \Cref{sec:continuity_eq})
\begin{equation}\label{eq:continuity_eq}
\frac{\partial \mu_t}{\partial t}+\divT(\mu_t v_t ) =0
\end{equation}
where $v_t$ should ensure the convergence of $\mu_t$ to $\pi$, for some topology over measures, in finite or infinite time.  Due to $v_t$, \cref{eq:continuity_eq} is nonlinear over $\mu_t$. Cauchy-Lipschitz-style assumptions for existence and uniqueness of the solution of \eqref{eq:continuity_eq} are provided in \Cref{sec:Cauchy-Lip_flow}. The continuity equation ensures that the mass is conserved and that it is not teleported as for a mixture $\mu_t=(1-t)\mu_0+t\pi$. In order to adjust the position of particles only depending on the present distribution $\mu_t$ and to have an automated choice of $v_t$ at any given time, it is favorable to have $v_t$ as a function of $\mu_t$, written as $v_{\mu_t}$.%, i.e.\ define $v_{\mu_t}$ in a closed-loop fashion.%\pab{I'd remove closed-loop if it is not used later}

%\pca{mention OT Benamou-brenier-Villani as finite time controllability whereas we do stabilization in infinite time}
%\subsection{Lyapunov analysis and gradient flows}
%\label{sec:sub_Lyap}
A principled way to select such a $v_{\mu_t}$ is to define it based on a Lyapunov functional $\cF(\mu)$ over measures, decreasing along the Wasserstein gradient flow (see \Cref{sec:W2_diff})
\begin{equation}\label{eq:Lyap_deriv}
 \dcF(\mu_t):=\frac{\d \cF(\mu_t)}{\d t}=\ps{\nabla_{W_2}\cF(\mu_t),v_{\mu_t}}_{L^2(\mu_t)}\le 0.
\end{equation}
Any dissimilarity $\cF(\cdot)=D(\cdot|\pi)$ is a valid Lyapunov candidate since it is non-negative and vanishes at $\pi$. Hence, \eqref{eq:continuity_eq} can be seen as a continuous descent scheme of \eqref{eq:min_D} or, conversely, \eqref{eq:min_D}-\eqref{eq:Lyap_deriv} can be interpreted as a way to choose $v_{\mu_t}$ in \eqref{eq:continuity_eq} to steer $\mu_0$ to $\pi$. In short, any Lyapunov-based approach rests upon three quantities ($\cF(\mu_t),v_{\mu_t},\dcF(\mu_t)$), related by \eqref{eq:Lyap_deriv}. A natural choice of $v_{\mu_t}$ satisfying \eqref{eq:Lyap_deriv} and realizing the steepest descent is the Wasserstein gradient itself, $v_{\mu_t}=-\nabla_{W_2}\cF(\mu_t)$. Depending on the choice of $\cF$, this $v_{\mu_t}$ may be hard to implement, or require specific analysis of the resulting dissipation function $\dcF(\mu_t)$. Otherwise, to ensure that $\dcF(\mu_t)$ only vanishes at $\pi$, one can choose $v_{\mu_t}$ so that both $\cF(\mu_t)$ and $\dcF(\mu_t)$ are known dissimilarities. As a matter of fact, if there exists a dissimilarity $\tilde{D}$ separating measures such that $-\dcF(\mu)\ge \tilde{D}(\mu|\pi)$, then $\pi$ is asymptotically stable for the flow and, if $\tilde{D}(\mu|\pi)\ge \cF(\mu)$, then $\pi$ is exponentially stable (by Gronwall's lemma). This relates the Lyapunov analysis to functional inequalities \cite{villani2003optimal}, expressing domination w.r.t.\ $\cF$ of the Wasserstein gradient of $\cF$ under specific assumptions on $\pi$, e.g.\ log-Sobolev for the KL, or Poincaré for the $\chi^2$ \cite{chewi2020svgd}.
%\pab{I feel like there is not enough connection with the rest}\pab{I feel like this paragraph is too abstract} 


%While any given closed-loop vector field $v_{t,\mu_t}$ can be compatible with several Lyapunov functionals\pab{compatible = decreases the functional? I'm not sure that anyone interested in the paper is super familar with Lyapunov functions, maybe explain a bit more}, it can only be the gradient of a single functional.\footnote{\pca{I dismiss constants because I ask them to vanish at $\pi$}} In order to leverage performing optimization algorithms, such as L-BFGS, it is beneficial to select a Lyapunov functional appropriate to the considered setting and set $v_t$ to be its Wasserstein gradient flow\pab{Why? I think that this is one of the key point of the paper, so it should be explained in more details. I htink that the use of L-BFGS is allowed because we have a tractable functional over discrete measures}. We thus propose to follow the Kernel Stein Discrepancy gradient flow\pab{I think that it should be introduced in a few words, and motivated: why use it? what does it bring to the table that other methods do not have?}.

%SVGD takes $\cF(\mu_t)$ to be the KL and $\dcF(t)$ as the KSD\pab{The KSD has never been introduced at this point}\pab{What does " $\dot F$ is the KSD" precisely mean?}. LAWGD takes $\cF(\mu_t)$ as the KL and $\dcF(t)$ as the $\chi^2$. The drawback of these approaches is that $\cF(\mu_t)$ is hard to compute\pab{I think that it should be stressed more that the KL cannot be evaluated easily from samples} and optimize over, so \eqref{eq:Lyap_deriv} is favoured over \eqref{eq:min_D}\pab{I don't understand what this last part means}.

%The choice of a given dissimilarity $D$ for $\cF$ is binding since it reverberates across both the underlying -stronger or weaker- topology over $\cP_2(\X)$ and the nature -deterministic or stochastic- of the associated gradient flow. For instance the KL divergence defines a strong topology, known to require equality of the measure supports, and defining few continuous losses \cite{arjovsky17GAN}, while the entropy term it contains entails Brownian dynamics. The choice of $D$ also depends on the available knowledge over $\pi$, for instance samples of $\pi$ for the MMD or a score function for the KSD.  Sometimes $\pi$ is also known only up to a normalizing constant, a.k.a. the partition function, which favors $\log \pi$-based dissimilarities such as the KL or the KSD.

%\section{Background on the Kernel Stein Discrepancy}

\subsection{Kernel Stein Discrepancy}\label{sec:background_ksd}

Consider a positive semi-definite kernel $k : \R^d \times \R^d \to \R$ and its corresponding RKHS $\cH_k$ of real-valued functions on %an open set $\X\subseteq $
$\R^d$. The space $\mathcal{H}_k$ is a Hilbert space with inner product $\ps{\cdot,\cdot}_{\cH_k}$ and norm $\Vert \cdot \Vert_{\cH_k}$. Moreover, $k$ satisfies the reproducing property: $
\forall \; f \in \cH_k,\; f(x)=\ps{f,k(x,\cdot)}_{\cH_k}$; which for smooth kernels also holds for derivatives, e.g.\ $\p_i f(x)=\ps{f,(\nabla_1 k(x,\cdot))_i}_{\cH_k}$ \citep[see][]{saitoh16theory}. Let $\mu \in \cP_2(\X)$. If $\int k(x,x) \d\mu(x)<\infty$, then the integral operator associated to the kernel $k$ and measure $\mu$, denoted by
$S_{\mu, k}: L^2(\mu) \rightarrow \Hk$ and defined as\vspace{-3mm}
\begin{equation}\label{eq:integral_operator}
S_{\mu, k}f  = \int k(x,\cdot)f(x)\d\mu(x),
\vspace{-3mm}
\end{equation}
is a Hilbert-Schmidt operator and $\Hk\subset L^2(\mu)$. In this case, the identity embedding $\iota:\Hk\to L^2(\mu)$ is a bounded operator and it is the adjoint of $S_{\mu,k}$ (i.e., $\iota^*=S_{\mu,k}$ \citep[Theorems 4.26 and 4.27]{steinwart2008support}. Hence, for any $(f,g)\in \Hk\times L^2(\mu)$, $\ps{\iota f,g}_{L^2(\mu)}=\ps{f,S_{\mu,k}g}_{\Hk}$.
We denote by $\cH_k^d$ the Cartesian product RKHS consisting of elements $f=(f_1, \dots, f_d)$ with $f_i\in \cH_k$, and with inner product $\ps{f,g}_{\cH_k^d}=\sum_{i=1}^d\ps{f_i,g_i}_{\cH_k}$.\ For vector-inputs, we extend $S_{\mu, k}$, applying it component-wise.

%The operator $S_{\mu,k}^\starS_{\mu,k}$ is compact, positive and self-adjoint 
%In the following, we will assume that $k$ is symmetric, translation invariant, and $C^{1,1}(\X \times \X)$. \pca{Do we ?}
%Notice that as soon as $k$ is translation invariant, we have $ \nabla_x k(x,y) = - \nabla_y k(x,y) = -\nabla_y k(y,x)$ and 
%the Stein kernel is symmetric as well. 
%under mild regularity assumptions on $k$ and $\pi$.\footnote{More precisely, $k\in C^{1,1}$, $\pi$ has a $C^1$-density and $\int_\X \nabla_x (k(x,y)\pi(x)) \d x=0$, see \citet[Theorem 3.7]{liu2016kernelized}.
The Stein kernel $\kpi$ \eqref{eq:stein_kernel} is a reproducing kernel and satisfies a Stein identity ($\int_{\X} \kpi(x,\cdot)\d\pi(x)=0$) under mild regularity assumptions on $k$ and $\pi$.\footnote{e.g., $k$ is a Gaussian kernel and $\pi$ is a smooth density fully supported on $\R^d$, see \citet[Theorem 3.7]{liu2016kernelized}.} It allows for several interpretations of the KSD \eqref{eq:ksd} as already discussed by \citet{liu2016kernelized}. It can be introduced as an IPM in the specific case of a Stein operator applied to $\Hk$ \citep[e.g.][]{gorham2017measuring}. It can then be identified as an asymmetric MMD in $\Hkpi$ (see \Cref{sec:related_work}). 
Alternatively, the squared KSD can be seen as a kernelized Fisher divergence, where the Fisher information $\| \nabla \log \left(\frac{\d\mu}{\d\pi}\right)\|^2_{L^2(\mu)}$ is smoothed through the kernel integral operator, i.e.\ $\KSD^2(\mu|\pi)= \|S_{\mu, k}\nabla \log\left(\frac{\d\mu}{\d\pi}\right)\|^2_{\cH^d_k}$. In this sense, the squared KSD has also been referred to as the Stein Fisher information \cite{duncan2019geometry}. Hence, minimizing the KSD can be thought as a kernelized version of score-matching \cite{hyvarinen2005estimation}.
%\ak{isn't it redondant with l148?} \pca{I did not say what the Stein operator was} %\pca{Missing, the Stein operator and its relation with diffusion}%\footnote{Notice that the above quantity is related to the classical relative Fisher information defined by $\| \nabla \log \left(\frac{\mu}{\pi}\right)\|^2_{L^2(\mu)}$. The latter corresponds to the squared $W_2$ gradient of the Kullback-Leibler divergence defined by $KL(\mu|\pi)=\int \log \left(\frac{d\mu}{d\pi}(x) \right) d\mu(x)$ if $\mu$ is absolutely continuous w.r.t. $\pi$ with Radon-Nikodym density $d\mu/d\pi$, and $KL(\mu|\pi) =+\infty$otherwise \citep[see][]{wibisono2018sampling}. } 

The metrization of weak convergence by the KSD, i.e.\ that %$\KSD(\mu_t|\pi) \to 0$ when $t\to \infty$ 
$\lim_{t\to \infty}\KSD(\mu_t|\pi) =0$ 
implies the weak convergence of $\mu_t$ to $\pi$, depends on the choice of the kernel relatively to the target. This question has been considered by~\citet{gorham2017measuring}, who show this is the case under assumptions akin to strong log-concavity of $\pi$ at infinity \citep[namely distant dissipativity,][]{eberle2016reflection}, and for a kernel $k$ with a slow decay rate. %Sufficient conditions include $\pi$ being distantly dissipative i.e.\ such that $ \lim \inf_{r \to \infty}   \kappa(r) > 0$ for $\kappa(r) =	\inf \{ -2 \ps{ \nabla \log \pi (x)- \nabla \log \pi(y),x-y }/\|x-y\|_2^2 ; \|x-y\|_2=r	\}$. 
This includes finite Gaussian mixtures with common covariance and %candidate 
kernels that are translation-invariant with heavy-tails and non-vanishing Fourier transform, such as the inverse multi-quadratic (IMQ) kernel defined by $k(x,y)=(c^2 + \|x- y\|_2^2)^{\beta}$ for $c >0$ and $\beta \in (-1, 0)$, or its variants considered in \citet{chen2018stein}. %and all distributions	strongly log-concave outside of a compact set. , includingBayesian linear, logistic, and Huber regression posteriorswith Gaussian priors. 
	 
%In these cases, the convergence of the $\KSD(\mu_t|\pi)$ to $0$ implies the weak convergence of $(\mu_t)$ to $\pi$.



%\subsection{KSD connection with other metrics}





==> KSD descent/experiments.tex <==

\section{Experiments}\label{sec:experiments}

%\ak{add complexity + time running to show efficiency of our approach, details of implementation}
%\ak{for the complexity, if we do stochastic descent (ie sample random pairs for the Ustat) can we gain a lot ofcomplexity compared to SVGD?}


In this section, we discuss the performance of KSD Descent to sample from $\pi$ in practice, on toy examples and real-world problems. The code to reproduce the experiments and a package to use KSD Descent are available at \url{https://github.com/pierreablin/ksddescent}. For all our experiments, we use a Gaussian kernel, as we did not notice any difference in practice w.r.t.\ the IMQ kernel. Its bandwith is selected by cross-validation. Implementation details and additional experiments can be found in \Cref{sec:more_experiments}.%The reader may refer to \Cref{sec:more_experiments} for i

\subsection{Toy examples}\label{sec:experiments_toy}

\begin{figure}
    \centering
    \includegraphics[width=.24\columnwidth]{figures/simple_gaussian_2d_svgd.pdf}
    \includegraphics[width=.24\columnwidth]{figures/simple_gaussian_2d_mmd.pdf}
    \includegraphics[width=.24\columnwidth]{figures/simple_gaussian_2d_grad.pdf}
    \includegraphics[width=.24\columnwidth]{figures/simple_gaussian_2d_bfgs.pdf}
    \caption{Toy example with 2D standard Gaussian. The green points represent the initial positions of the particles. The light grey curves correspond to their trajectories under the different $v_{\mu_t}$.}% vector fields
    \label{fig:toy_example}
\end{figure}
%We first consider some toy examples. 
In the first example, we choose $\pi$ to be a standard 2D Gaussian, and a Gaussian $k$ with unit bandwidth. We initialize with $50$ particles drawn from a Gaussian with mean $(1,1)$.
\Cref{fig:toy_example} displays the trajectories of several different methods: SVGD, KSD Descent implemented using gradient descent (\Cref{alg:ksd_descent_GD}) and L-BFGS (\Cref{alg:ksd_descent_LBFGS}), and the MMD flow \cite{arbel2019maximum}. To assess the convergence of the algorithms, for SVGD we monitored the norm of the displacement, while for the KSD and MMD gradient flows we used the tolerance parameter of L-BFGS. KSD Descent successfully pushes the particles towards the target distribution, with a final result that is well-distributed around the mode. %It appears to be robust even when the particles are initialized further from the target $\pi$.
%\ak{bonus: a figure that shows the initialized particles: that show that even if we initialize far from the target we converge.}\pab{In that regard we are worse than SVGD}
While KSD performs similarly to SVGD, we can notice that the trajectories of the particles behave very differently. Indeed, SVGD trajectories appear to be at first driven by the score term in the update, while the repulsive term acts later to spread the particles around the mode. In contrast, trajectories of the particles updated by KSD Descent are first influenced by the last repulsive term of the update, which seems to determine their global layout, and are then translated and contracted towards the mode under the action of the driving terms. Finally, for the MMD descent, some particles collapse around the mode, while others stay far from the target. This behavior was documented in~\citet{arbel2019maximum}, and can be partly circumvented by injecting some noise in the updates.
% This phenomenon might be explained by the difference in the repulsive terms in KSD Descent and SVGD \ak{should we write the repulsive terms for both? we can show the landscape for both terms maybe}\pab{Not in 2d :(}.
 
 \begin{figure}
    \centering
    \includegraphics[width=.99\columnwidth]{figures/convergence_speed.pdf}
    \caption{Convergence speed of KSD and SVGD on a Gaussian problem in 1D, with 30 particles.}
    \label{fig:conv_speed}
\end{figure}
 
 We then compare the convergence speed of KSD Descent and SVGD in terms of the KL or KSD objective (see \Cref{fig:conv_speed}). With a fine-tuned step-size, SVGD is the fastest method. However, taking a step-size too large leads to non-convergence, while one too small leads to slow convergence. It should be stressed that it is hard to select a good step-size, or to implement a line-search strategy, since SVGD does not minimize a simple function. In contrast,
 the empirical KSD \eqref{eq:discrete_loss} can be minimized using L-BFGS, which does not have any critical hyper-parameter.%\ak{apart the bandwith of the kernel for both.}\pab{Yes but this is not an 'optim' hyperparameter. Also this means that SVGD in fact has 2 hyperparameters, which is really bad: 2 hyperparameters is much much worse than one.}
 
\begin{figure}
    \centering
    \includegraphics[width=.48\columnwidth]{figures/bad_minima_init2.pdf}
    \includegraphics[width=.48\columnwidth]{figures/bad_minima_init1.pdf}
    \caption{KSD Descent applied on a balanced mixture of Gaussian with small variance (0.1) in 2D. The centroids are at $(-1, 0)$ and $(1, 0)$. The green crosses indicate the initial particle positions, while the blue ones are the final positions. The light red arrows correspond to the score directions. \textbf{Left}: the initial positions are all chosen close to the line $x=0$, which corresponds to an axis of symmetry of $\pi$. \textbf{Right}: even when the initialization is more spread, some particles are still caught in this spurious local minimum.}%line where the score is stable\ak{stable?}\pab{We should use the same term as in prop.3
    \label{fig:mog_problem}
\end{figure}
 In our second example, we apply KSD Descent for $\pi$ taken as a symmetric mixture of two Gaussians with the same variance. This highlights the results of \Cref{sec:spurious_minima}. If initialized on the axis of symmetry, the particles are indeed stuck on it, as stated in \Cref{lem:Flow-invariant symmetry}. We noticed that, for a large variance of $\pi$ (e.g.\ in $[0.2,1]$), this axis is unstable. However, when the variance is too small (e.g.\ set to 0.1 as in \Cref{fig:mog_problem}), the axis can even become a locally stable set. We also observed that, for a distribution initialized exclusively on one side of the axis, a single component of the mixture can be favored. This is a classical behavior of score-based methods, depending typically on the variance of $\pi$ \cite{wenliang2020blindness}.%\pca{J'ai déplacé ci-dessous la modif de qqun avec laquelle je ne suis pas d'accord.}
 
 %Indeed, when the variance of the gaussians is too small (e.g.\ set to 0.1 as on \Cref{fig:mog_problem}), the axis of symmetry can  become a locally stable set. If initialized on the axis of symmetry, the particles are indeed stuck on it, as stated in \Cref{lem:Flow-invariant symmetry}. We noticed that, for a large variance of $\pi$ (e.g.\ in $[0.2,1]$), this axis is an unstable set. We also observed that, for a distribution initialized exclusively on one side of the axis, a single component of the mixture can be favored. This is a classical behavior of score-based methods when the variance is too small \cite{wenliang2020blindness}. % converge to a local minimum on the axis of symmetry of the target. %As predicted by \Cref{sec:spurious_minima}, the particles are converging to a spurious local minimum.

To fix this issue, we consider an annealing strategy as suggested by \citet{wenliang2020blindness}. It consists in adding an inverse temperature variable $\beta$ to the log density of the model, i.e.\ $\pi^{\beta}(x)\propto \exp(-\beta V(x))$ for $\pi(x)\propto \exp(-V(x))$, with $\beta \in (0, 1]$. This is easily implemented with score-based methods, since it simply corresponds to multiplying $s(x)$ by $\beta$. When $\beta$ is small, annealing smoothes the target distribution and the last term of the Stein kernel, repulsive at short distance, becomes dominant; on the other hand, for $\beta$ close to 1, we recover the true log density. To implement this method, we start with $\beta=0.1$, and run the KSD Descent to obtain particles at `high temperature`. KSD Descent is then re-run starting from these particles, setting now $\beta = 1$. One can see that this strategy successfully solves the issues encountered when the KSD flow was failing to converge to the target $\pi$ (\Cref{fig:toy_example_annealing}).
This correction differs from the noise-injection strategy proposed in \citet{arbel2019maximum} for the MMD flow, which is rather related to randomized smoothing \cite{duchi2012randomized}. Noise-injection would prevent the use of L-BFGS in our case, as it requires exact values of the gradients of previous iterations. Annealing on the other hand is compatible with \Cref{alg:ksd_descent_LBFGS}. %\pab{we might talk about it before when the issue arises in the first figure?} However, %which consists in injecting noise on the positions of the particles where the gradient is evaluated, a strategy often to referred as

\begin{figure}
    \centering
    \includegraphics[width=.32\columnwidth]{figures/temperature_direct.pdf}
    \includegraphics[width=.32\columnwidth]{figures/temperature_hightemp.pdf}
    \includegraphics[width=.32\columnwidth]{figures/temperature_lowtemp.pdf}
     \caption{Effect of the annealing strategy on a mixture of Gaussians. \textbf{Left}: without annealing, some particles fall into a spurious minimum. \textbf{Middle}: with a higher temperature ($\beta = 0.1$), the particles are more spread out. \textbf{Right}: starting from the particles in the middle figure and setting $\beta=1$ we converge to a distribution which minimizes the KSD, and has no spurious particles.}
    \label{fig:toy_example_annealing}
\end{figure}
\subsection{Bayesian Independent Component Analysis}
Independent Component Analysis \citep[ICA,][]{comon1994independent} is the generative model $x = W^{-1}s$, where $x$ is an observed sample in $\R^p$, $W\in\R^{p\times p}$ is the unknown square unmixing matrix, and $s\in\R^p$ are the independent sources. We assume that each component has the same density $s_i \sim p_s$. The likelihood of the model is $p(x|W) = \log|W| + \sum_{i=1}^pp_s([Wx]_i)$. For our prior, we assume that $W$ has i.i.d.\ entries, of law $\mathcal{N}(0, 1)$. The posterior is $p(W|x) \propto p(x|W)p(W)$, and the score is given by $s(W) = W^{-\top} - \psi(Wx)x^{\top} - W$, where $\psi = - \frac{p'_s}{p_s}$.
In practice, we choose $p_s$ such that $\psi(\cdot) = \tanh(\cdot)$.
We then use the presented algorithms to draw particles $W\sim p(W|x)$.
%
We use $N = 10$ particles, and take $1000$ samples $x$ from the ICA model for $p\in\{2,4,8\}$.
%
Each method outputs $N$ estimated unmixing matrices, $[\tilde{W}_i]_{i=1}^N$.
%, $i=1\dots N$
We compute the Amari distance~\citep{amari1996new} between each $\tilde{W}_i$ and $W$: the Amari distance vanishes if and only if the two matrices are the same up to scale and permutation, which are the natural indeterminacies of ICA.
We repeat the experiment $50$ times, resulting in $500$ values for each algorithm (\Cref{fig:ica}). We also add the results of a random output, where the estimated matrices are obtained with i.i.d.\ $\mathcal{N}(0, 1)$ entries.
\begin{figure}
    \centering
    \includegraphics[width=.32\columnwidth]{figures/ica_2.pdf}
    \includegraphics[width=.32\columnwidth]{figures/ica_4.pdf}
    \includegraphics[width=.32\columnwidth]{figures/ica_8.pdf}
    \caption{Bayesian ICA results. Left: $p=2$. Middle: $p=4$. Right: $p=8$. Each dot corresponds to the Amari distance between an estimated matrix and the true unmixing matrix.}
    \label{fig:ica}
\end{figure}
We see that for this experiment, KSD performs barely better than random, while SVGD finds matrices with lower Amari distance.
%
One explanation is that the ICA likelihood is highly non-convex~\citep{cardoso1998blind}. This is easily seen with the invariances of the problem: permuting the rows of $W$ does not change $p(x|W)$. As a consequence, the posterior has many saddle points, in which particles might get trapped. Unfortunately, the annealing strategy proposed above did not improve the achieved performance for this problem.%, as it performs equally poorly.

%
%As a consequence, there are many $W$ such that $s(W) = 0$ but for which $W$ is not a local maximum of the likelihood. These spurious points are attractive for the KSD algorithm.\pab{Actually I have checked: KSD finds points with a non zero score norm...}

\subsection{Real-world data}

We compare KSD Descent and SVGD in the Bayesian logistic regression setting described in \citet{gershman2012nonparametric, liu2016stein}. Given datapoints $d_1, \dots, d_q \in \R^p$, and labels $y_1, \dots, y_q\in \{\pm 1\}$, the labels $y_i$ are modelled as $p(y_i = 1| d_i, w) = (1 + \exp(-w^{\top}d_i))^{-1}$ for some $w\in \R^p$. The parameters $w$ follow the law $p(w |\alpha) = \mathcal{N}(0, \alpha^{-1}I_p)$, and $\alpha > 0$ is drawn from an exponential law $p(\alpha) = \mathrm{Exp}(0.01)$. The parameter vector is then $x = [w, \log(\alpha)] \in \R^{p+1}$, and we use \Cref{alg:ksd_descent_LBFGS} to obtain samples from $p(x| \left(d_i, y_i)_{i=1}^q\right)$ for $13$ datasets, with $N=10$ particles for each.

The learning rate for SVGD and the bandwidth of the kernel for both methods are chosen through grid-search, and for each problem we select the hyper-parameters yielding the best test accuracy. For all problems, the running times of SVGD with the best step-size and of KSD Descent were similar, while KSD Descent has the advantage of having one less hyper-parameter. We present on \Cref{fig:logreg} the accuracy of each method on each dataset, where KSD Descent was applied without annealing since it did not change the numerical results. Our results show we match the SVGD performance without having to fine-tune the step-size, owing to \Cref{alg:ksd_descent_LBFGS}.
%
We posit that KSD succeeds on this task because the posterior $p(x| \left(d_i, y_i)_{i=1}^q\right)$ is log-concave, and does not have saddle points.
%Our results are very comparable to the ones of the SVGD algorithm, with an improvement of $2\%$ on one of the 13 datasets.


\begin{figure}[ht]
    \begin{minipage}[c]{0.45\linewidth}
        \includegraphics[width=\textwidth]{figures/logreg.pdf}
    \end{minipage}\hfill
    \begin{minipage}[c]{0.45\linewidth}
        \vspace{-1em}
    \caption{Accuracy of the KSD Descent and SVGD on bayesian logistic regression for 13 datasets. Both methods yield similar results. KSD is better by $2\%$ on one dataset.}\label{fig:logreg}
    \end{minipage}
    \vspace{-1em}
\end{figure}

==> KSD descent/method.tex <==

\section{Sampling as optimization of the KSD}\label{sec:ksd_descent}


%\subsection{Kernel Stein Discrepancy Descent}


This section defines the KSD Descent and relates it to other gradient flows, especially the MMD gradient flow, of which the KSD Descent is a special case. In all the following, we assume that $k\in C^{3,3}(\R^d\times \R^d, \R)$, and that $\pi$ is such that $s=\nabla\log\pi\in C^2(\R^d)$.


\subsection{Continuous time dynamics}

Consider the functional
$\cF : \cP_2(\X) \to [0,+\infty)$, $\mu \mapsto \frac{1}{2}\KSD^2(\mu|\pi)$  %$\cF : \cP_2(\X) \to (-\infty,+\infty]$ 
defined over the Wasserstein space. 
If $\mu \in \cP_2(\X)$ satisfies some mild regularity conditions (i.e., it has a $C^1$ density w.r.t. Lebesgue measure, and it is in the domain of $\cF$, see \Cref{sec:W2_diff}), the  gradient of $\cF$ at $\mu$ is well-defined and denoted by $\nabla_{W_2} \cF(\mu) \in L^2(\mu)$. We shall consider the following assumptions on the Stein kernel:
\vspace{-0.15cm}
\newcounter{contlist}
\begin{assumplist}
	\setlength\itemsep{0.2em}
	\item \label{ass:lipschitz} There exists a map $L(\cdot)\in C^0(\X,\R_+)$, which is $\mu$-integrable for any $\mu \in \cP_2(\X)$, such that, for any $y \in \X$, the maps $x\mapsto \nabla_1 \kpi(x,y)$ and $x\mapsto \nabla_2 \kpi(x,y)$ are $L(y)$-Lipschitz. 
	\item \label{ass:growth} There exists $m>0$ such that for any $\mu \in \cP_c\left(\R^{d}\right),$ for all $y \in \R^{d},$ we have $\|\int \nabla_2 k_{\pi}(x,y) \d\mu(x)\| \leq m\left(1+\|y\|+\int \|x\|\,\d\mu(x)\right).$
	%$y\mapsto \nabla_2 k_{\pi}(x,y)$ is Lipschitz with constant $L>0$.
	\item \label{ass:square_der_int} The map $(x,y) \mapsto \|H_1 \kpi(x,y)\|_{op}$ is $\mu\otimes\nu$-integrable for every $\mu,\nu\in \cP_2(\X)$.
	\item \label{ass:integrable} For all $\mu\in \cP_2(\X)$, $\int \kpi(x,x)\d\mu(x)<\infty$.
\end{assumplist}
\vspace{-0.15cm}
The KSD gradient flow is defined as the flow induced by the continuity equation:
\begin{equation}\label{eq:ksd_flow}
\frac{\partial \mu_t}{\partial t}+\divT(\mu_t v_{\mu_t} ) =0 \text{ for } v_{\mu_t} := - 
\nabla_{W_2}\cF(\mu_t).
\end{equation}
\Cref{ass:lipschitz,ass:growth} ensure that the KSD gradient flow exists and is unique, they are further discussed in \Cref{sec:Cauchy-Lip_flow}. \Cref{ass:lipschitz,ass:square_der_int} are needed so that the Hessian of $\cF$ is well defined (see \Cref{sec:convergence}). \Cref{ass:integrable} guarantees that the integral operator $S_{\mu, \kpi}$ \eqref{eq:integral_operator} is well-defined and that $\cF(\mu)<\infty$ for all $\mu\in \cP_2(\X)$.
\begin{lemma}\label{lem:lipschitz_ass}
	 Assume that $k$, its derivatives up to order 3, and their product by $\|x-y\|$ are uniformly bounded over $\X$; and that $s$ is Lipschitz and has a bounded Hessian over $\X$. Then \Cref{ass:lipschitz,ass:square_der_int,ass:integrable} hold. If, furthermore there exists $M>0$ and $M_0$ such that, for all $x\in\X$, $\|s(x) \|\le M\sqrt{\|x\|}+M_0$, then \Cref{ass:growth} also holds.
\end{lemma}
See the proof in \Cref{sec:proof_lem_lipschitz_ass}. Smoothed Laplace distributions $\pi$ paired with Gaussian $k$ satisfy the assumptions of \Cref{lem:lipschitz_ass}. For Gaussian $\pi$, $s$ is linear, so \Cref{ass:lipschitz,ass:square_der_int,ass:integrable} hold for smooth kernels, but \Cref{ass:growth} does not hold in general because of the $s(x)^\top s(y)$ term in $\kpi$. Notice that most of our results are stated without \Cref{ass:growth}, which is only required to establish the global existence of KSD flow, in the sense that the particle trajectories are well-defined and do not explode in finite-time.
 
\begin{proposition}\label{prop:dissipation}%\ak{write that it only holds for C1 densities} %\label{prop:W2_grad_KSD}
Under \Cref{ass:lipschitz,ass:growth}, the $W_2$ gradient of $\cF$ evaluated at $\mu$ and its dissipation \eqref{eq:Lyap_deriv} along \eqref{eq:ksd_flow} are
\begin{align}
\nabla_{W_2}\cF(\mu)&=\mathbb{E}_{x \sim \mu}[\nabla_{2}\kpi(x,\cdot)],\label{eq:ksd_w2_grad}\\
\dot{\cF}(\mu_t)&=-\E_{y\sim \mu_t}\left[ \| \mathbb{E}_{x \sim \mu_t}[\nabla_{2}\kpi(x,y)] \|^2\right] \label{eq:dissipation}.
\end{align}
\end{proposition}\vspace{-3mm}
Since the r.h.s. of \eqref{eq:dissipation} is negative, \Cref{prop:dissipation} shows that the squared KSD w.r.t.\ $\pi$ decreases along the KSD gradient flow dynamics. In other words, $\cF$ is indeed a Lyapunov functional for the dynamics \eqref{eq:ksd_flow} as discussed in \Cref{sec:sub_Lyap}.

%\begin{lemma}\label{lem:lipschitz_ass}
%	Assume $s$ is Lipschitz over $\X$. Assume $k$ and its  derivatives are bounded over $\X$. Assume also that $g_1:x\mapsto \| \nabla_2 k(x,y)\|$ and $g_2 : x \mapsto\| \nabla_2 ( \div_{2}\nabla_{2}k(x,y)\|$, are $g(y)$-Lipschitz where $g:y\mapsto C_1\|y\|+C_2$, which  holds for a Gaussian kernel for instance. Then \Cref{ass:lipschitz,ass:integrable} hold.
%\end{lemma}
%
%\begin{lemma}\label{lem:hessian_kpi}
%	Assume that $k$ and its derivatives up to order 3 are bounded over $\X$, and that $s\in C^2(\R^d)$ has a bounded Hessian. Then \Cref{ass:square_der_int} holds.
%\end{lemma}
\subsection{Discrete time and discrete measures}

A straightforward time-discretization of \eqref{eq:ksd_flow} is a gradient descent in the Wasserstein space applied to ${\cF(\mu)=\frac{1}{2}\KSD^2(\mu|\pi)}$. Starting from an initial distribution $\mu_0 \in \cP_2(\X)$, it writes as follows at iteration $n\in \N$,
\begin{equation}\label{eq:ksd_descent}
    \mu_{n+1} = \left(I -\gamma \nabla_{W_2} \cF(\mu_n)\right)_{\#} \mu_n,
\end{equation}
for a step-size $\gamma>0$. However for discrete measures $\hat{\mu}=\frac{1}{N}\sum_{j=1}^{N}\delta_{x^{j}}$, we can make the problem more explicit setting a loss function
\begin{equation}
    F([x^j]_{j=1}^{N}) :=%\frac{1}{2} \KSD^2(\hat{\mu}|\pi)
    \cF(\hat{\mu})
    =\frac1{2N^2}\sum_{i, j=1}^N\kpi(x^i, x^j).
    \label{eq:discrete_loss}
\end{equation}
Problem \eqref{eq:min_D} then corresponds to a standard non-convex optimization problem over the finite-dimensional, Euclidean, space of particle positions. The gradient of $F$ is readily obtained as\vspace{-2mm}
\begin{equation*}
     \nabla_{x^i} F([x^j]_{j=1}^{N}) = \frac{1}{N^2}\sum_{j=1}^N \nabla_{2}\kpi( x^{j},x^{i}).
\end{equation*}
since, by symmetry of $\kpi$, $\nabla_1\kpi(x,y)=\nabla_2\kpi(y,x)$. As both $F$ and $\nabla_{x^i} F$ can be explicitly computed, one can implement the KSD Descent either using a gradient descent (\Cref{alg:ksd_descent_GD}) or through a quasi-Newton algorithm such as L-BFGS (\Cref{alg:ksd_descent_LBFGS}). As a matter of fact, L-BFGS \cite{liu1989limited} is  often faster and more robust than the conventional gradient descent. It also does not require choosing critical hyper-parameters, such as a learning rate, since L-BFGS performs a line-search to find suitable step-sizes. It only requires a tolerance parameter on the norm of the gradient, which is in practice set to machine precision.
%In practice, initializing with $N$ i.i.d.\ samples $x_0^{i}\sim \mu_0$, the KSD Descent updates the positions of the $N$ particles. 
%\pab{The algorithm for KSD Descent is not exactly what we do, because we do a gradient descent (all particles updated at once, not one by one)}
\begin{algorithm}[ht]
   \caption{KSD Descent GD}
   \label{alg:ksd_descent_GD}
\begin{algorithmic}
   \STATE {\bfseries Input:} initial particles $(x_0^i)_{i=1}^{N}\sim \mu_0$, number of iterations $M$, step-size $\gamma$
   \FOR{$n=1$ {\bfseries to} $M$}
   %\FOR{$i=1$ {\bfseries to} $N$}
   \STATE
      \vspace{-0.8cm}
{\begin{equation}\label{eq:ksd_update}
    \hspace{-0.5cm}[x_{n+1}^{i}]_{i=1}^{N}=[x_n^{i}]_{i=1}^{N} - \frac{\gamma}{N^2}\sum_{j=1}^N [\nabla_{2}\kpi( x_n^{j},x_n^{i})]_{i=1}^{N},
    \end{equation}}
   \vspace{-0.8cm}
    %\ENDFOR
   \ENDFOR
   \STATE \textbf{Return: }$[x_{M}^i]_{i=1}^{N}$.
   \end{algorithmic}
\end{algorithm}
\begin{algorithm}[ht]
   \caption{KSD Descent L-BFGS}
   \label{alg:ksd_descent_LBFGS}
\begin{algorithmic}
   \STATE {\bfseries Input:} initial particles $(x_0^i)_{i=1}^{N}\sim \mu_0$, tolerance $\mathrm{tol}$
   \vspace{0.2cm}
   \STATE \textbf{Return: }$[x_*^i]_{i=1}^{N} = \mathrm{L}\text{-}\mathrm{BFGS}(F, \nabla F, [x_0^i]_{i=1}^{N}, \mathrm{tol})$.
    %\vspace{0.2cm}
     %\STATE \textbf{Return : }$[x_*^i]_{i=1}^{N}$.
    \end{algorithmic}
\end{algorithm}
A technical descent lemma for \eqref{eq:ksd_descent} (\Cref{prop:descent_lemma_appendix}) showing that $\cF$ decreases at each iteration \eqref{eq:ksd_descent} is provided in \Cref{sec:descent_lemma}. It requires the boundedness of $(\|L(\cdot)\|_{L^2(\mu_n)})_{n\ge0}$, the $L^2$-norm of the Lipschitz constants of \Cref{ass:lipschitz} along the flow, as well as the convexity of $L(\cdot)$ and a compactly-supported initialization.

\begin{remark}
As L-BFGS requires access to exact gradients, \Cref{alg:ksd_descent_LBFGS} cannot be used in a stochastic setting. However this can be done for \Cref{alg:ksd_descent_GD} by subsampling over particles in the double sum in \Cref{eq:discrete_loss}. Moreover, in some settings like Bayesian inference, the score itself writes as a sum over observations. In this case, the loss $F$ writes as a \emph{double} sum over observations, and a stochastic variant of \Cref{alg:ksd_descent_GD} tailored for this problem could be devised, in the spirit of~\citet{clemenccon2016scaling}. 
\end{remark}


\subsection{Related work}\label{sec:related_work}
%\pca{Ajouter non-asymptotic SVGD}%ak : done below
Several recent works fall within the framework sketched in Section \ref{sec:sub_Lyap}. In SVGD, \citet{liu2016kernelized} take $\cF$ as the KL, and set $v_{\mu_t}=-S_{\mu, k}\nabla\ln\left(\frac{d\mu_t}{d\pi}\right)$ to obtain $\dcF$ as the (squared) KSD. Integrating this inequality w.r.t. time yields a $1/T$ convergence rate for the average $\KSD$ between $\mu_t$ and $\pi$ for $t\in [0,T]$. This enabled \citet[Proposition 5, Corollary 6]{korba2020non} to obtain a discrete-time descent lemma for bounded kernels, as well as rates of convergence for   
the averaged $\KSD$. In contrast, since the dissipation \eqref{eq:dissipation} of the $\KSD$ along its $W_2$ gradient flow does not correspond to any dissimilarity, our descent lemma for \eqref{eq:ksd_descent} (\Cref{prop:descent_lemma_appendix}) does not yield similar rates of convergence.
Alternatively, in the LAWGD algorithm recently proposed by \citet{chewi2020svgd}, $\cF$ is the KL, and $v_{\mu_t}=-\nabla S_{\pi, k_{\cL_\pi}}\left(\frac{d\mu_t}{d\pi}\right)$ with $k_{\cL_\pi}$ chosen such that $\dcF$ is the $\chi^2$, by taking $S_{\pi, k_{\cL_\pi}}$ as the inverse of the diffusion operator:
\begin{equation}\label{eq:def_diffusion_op}
    \cL_\pi : f\mapsto-\Delta f-\langle \nabla \log\pi,\nabla f \rangle.
\end{equation}
%$\cL_\pi$ \eqref{eq:def_diffusion_op}
Their elegant approach results in a linear convergence of the KL along their flow, but implementing LAWGD in practice requires to compute the spectrum of $\cL_\pi$. It is in general as difficult as solving a linear PDE, and \citet{chewi2020svgd} admit it is unlikely to scale in high dimensions.\footnote{The update rules of SVGD, LAWGD and MMD-GD can be found in \Cref{sec:updates_related_work}.}% Originally kernels where meant to bypass Green functions by picking off-the-shelf kernels rather than solving PDEs. Applicability of reproducing kernels in machine learning mainly stems from implicit features maps.%\ak{this sentence waw more clear before i think}
%This is in line with viewing kernels as operators. 

Beyond studies on the KL, \citet{mroueh2019sobolev} considered $\cF$ as the MMD and pick $v_{\mu_t}$ based on a kernelized Sobolev norm so that $\dcF$ resembles the MMD, but without proving convergence of their scheme. \citet{arbel2019maximum} also analyzed $\cF$ as the MMD, but for $v_{\mu_t}=-\nabla_{W_2}\frac{1}{2}\MMD^2(\mu_t,\pi)$ with similar $\dcF$ as ours and with a dedicated analysis of their MMD-GD flow. We recall that $\MMD^2(\mu,\pi)=\|\int k(x,\cdot)d\mu(x)-\int k(x,\cdot)d\pi(x)\|_{\cH_k}^2$.
Since the Stein kernel satisfies the Stein's identity $\int \kpi(x,\cdot)d\pi(x)=0$, the KSD  \eqref{eq:ksd} can be identified to an MMD with the Stein kernel \cite{chen2018stein}. However, the assumptions of \citet{arbel2019maximum} -$\nabla k$ is $L$-Lipschitz for $L\in \R^+$- do not hold in general for unbounded Stein kernels. Here, we provide the right set of assumptions~\ref{ass:lipschitz}-\ref{ass:growth} on $\kpi$ for the flow to exist and for a descent lemma to hold. Also, as noted on \Cref{fig:toy_example}, the sample-based MMD flow, defined through
\begin{multline}\label{eq:mmd_grad}
    \nabla_{W_2}\frac{1}{2}\MMD^2(\mu,\pi)= \int \nabla_{2}k(x,\cdot) \d(\mu-\pi)(x)%\\    - \int \nabla_{2} k(x,.)d\pi(x)
\end{multline}
can fail dramatically while KSD flow succeeds. % Notice that the MMD flow also requires samples of $\pi$ to approximate \eqref{eq:mmd_grad}. 
%and in practice, as already noticed by \citet{arbel2019maximum}, MMD flow fails dramatically, even to approximate a simple Gaussian distribution as illustrated on \Cref{fig:toy_example}, e.g.\ when using a Gaussian kernel. %A large fraction of the particles crashes onto the mode, while some others are pushed far from $\pi$ and from the other particles. 
%In contrast, the score-based KSD flow successfully converge. 
This suggests that the geometrical properties of the KSD flow are more favorable than the ones of the regular MMD flow. In other words, choosing an appropriate (target-dependent) kernel, as in our method or in LAWGD, appears more propitious than %simply
taking a %general
kernel $k$ unrelated to $\pi$.


Related to the optimization of the $\KSD$, Stein points~\citep{chen2018stein} also propose to use the KSD loss for sampling, but the loss is minimized using very different tools. While KSD descent uses a first order information by following the gradient (or L-BFGS) direction with a fixed number of particles, Stein points use a Frank-Wolfe scheme, adding particles one by one in a greedy fashion. Given $N$ particles $x^1, \dots, x^N$, in Stein points, the next particle is set as
$$
x^{N+1} \in \argmin_{x} \frac12k_{\pi}(x, x) + \sum_{i=1}^N k_{\pi}(x, x^i).
$$
This problem is solved using derivative-free (a.k.a. zeroth-order) algorithms like grid-search or random sampling. The main drawback of such an approach is that it scales poorly with the dimension $d$ when compared to first-order methods. In the same spirit, \cite{futami2019bayesian} have recently proposed a similar algorithm to optimize the MMD.


%. 
%From a computational viewpoint both SVGD, LAWGD and MMD-GD only propose gradient descent schemes with the following respective updates $x_n^i \leftarrow x_n^i - \gamma \mathcal{D}^i$ with% where $\mathcal{D}$ is a $d \times N$ matrix with \pca{check the updates-move to appendix?}
%\begin{align*}
%    &\cD_{SVGD}^i = \frac1N\sum_{j=1}^N\left[k(x_n^j, x_n^i)s(x_n^j) + \nabla_{1} k(x_n^j, x_n^i)\right],\\
%    &\cD_{LAWGD}^i = \frac{1}{N}\sum_{j=1}^N \nabla_{2}k_{\cL_\pi}( x_n^{j},x_n^{i}),\\
%    &\cD_{MMD-GD}^i =\frac{1}{N}\sum_{j=1}^{N}\left[\nabla_2 k(x_{n}^{j}, x_{n}^{i})-\nabla_2 k(y^{j}, x_{n}^{i})\right].
%\end{align*}
%where the MMD-GD update requires extra samples $(y^{j})_{j=1}^N\sim \pi$, since it is sample-based rather than score-based. Notice that all these updates have the same iteration complexity of order $\mathcal{O}(N^2)$. Intriguingly LAWGD has the same update rule as ours \eqref{eq:ksd_update} but for their kernel $k_{\cL_\pi}$ which, as discussed above, does not incorporate an off-the-shelf kernel $k$, unlike \eqref{eq:stein_kernel}. 

%The great advantage of our formulation is that in the discrete case, corresponds to minimizing a simple cost function $\cL$ of the particles $(x^i)_{i=1}^{N}$, in contrast with SVGD and LAWGD (see \Cref{sec:related_work}).

%The operator $\mathcal{D}$ does not have a symmetric Jacobian\ak{ref?}, consequently SVGD iterations do not correspond to the gradient descent of some function over the particles $(x^i)_{i=1}^N$.
%Since we do not have a discrete Lyapunov function for the SVGD iterations, it is for instance impossible to implement a line-search technique to find a good step size. The performance of SVGD may vary importantly, see \Cref{fig:conv_speed}.

%\subsection{KSD Descent as an improved MMD Descent}\label{sec:ksd_mmd}
%We recall that $MMD^2(\mu,\pi)=\iint k(x,y) d\mu(x)d\mu(y) + \iint k(x,y)d\mu(x)d\mu(y) -2 \iint k(x,y) d\mu(x)d\mu(y)$.  

% Hence, our approach benefits from the following property, already proven in \citet{arbel2019maximum}. It is a descent result in discrete time, which shows that the KSD gradient flow decreases at each iteration and which holds for both continuous or discrete initializations.%under \Cref{ass:lipschitz}, under this assumption.% They are recalled here for completeness.theoretical guarantees

%\begin{proposition}\cite{arbel2019maximum}\label{prop:descent_lemma} Let $\mu_n$ be defined by \eqref{eq:ksd_descent}.
%Under \Cref{ass:lipschitz}, and for $\gamma \le \frac{2}{L}$, the sequence $(\cF(\mu_n))_{n\ge 0}$ is decreasing and for any $n\ge0$:
%\begin{equation*}%\label{eq:descent_lemma}
%    \cF(\mu_{n+1}) - \cF(\mu_n) \le -\gamma(1 - \frac{\gamma L}{2})  \|\nabla_{W_2}\cF(\mu_n)\|^2_{L^2(\mu_n)}.
%\end{equation*}
%\E_{x\sim \mu_n}[\nabla_2 \kpi(x,y)]
%\end{proposition}
%\pab{what is L? does it exist ? what happens in the continuous limit?}

%\Cref{prop:descent_lemma} states a descent result in discrete time, which shows that the KSD gradient flow decreases at each iteration. It holds for both continuous or discrete initializations. %In practice, if chosen continuous, $\mu_0$ is approximated by i.i.d.\ samples, which determine the empirical distribution $\hat{\mu}_0$ used in \Cref{alg:ksd_descent_GD}.% for an infinite number of particles, since it requires the knowledge of $\mu_n$

%\begin{proposition}\cite{arbel2019maximum}
%\label{prop:finite_particle}
%	Let $n\ge 0$ and $T>0$. Let $\mu_n$ and $\hat{\mu}_n$ be defined by \eqref{eq:ksd_descent} with initialization $\mu_0$ and $\hat{\mu}_0=\frac{1}{N}\sum_{i=1}^{N}\delta_{x_0^{i}}$ respectively, with $(x_0^i)_{i=1}^{N} \sim \mu_0$. Under \Cref{ass:lipschitz} for any $0\le n \le \frac{T}{\gamma}$:
%	\begin{equation*}
%	\E_{(x_0^i) \sim \mu_0}[W_2^2(\mu_n,\hat{\mu}_n)]\le \frac{e^{2LT}-1}{2\sqrt{N}} e^{LT}\sqrt{var(\mu_0)}. 
%	\end{equation*}
%%	where $L$ is a constant depending on $\kpi$ and $\pi$.
%\end{proposition}
%\Cref{prop:finite_particle} provides an upper bound of the finite-time deviation of the discrete distributions generated by \Cref{alg:ksd_descent_GD} for a finite number of particles from its population version $\mu_0$.% when the number of particles grow to infinity.

%Since it is sample-based, the implementation of the MMD-GD scheme  requires to have access to samples of $\pi$. However, as already noticed by \citet{arbel2019maximum}, it fails dramatically, even to approximate a simple Gaussian distribution as illustrated on \Cref{fig:toy_example}, e.g. when using a Gaussian kernel. A large fraction of the particles crashes onto the mode, while some others are pushed far from $\pi$ and from the other particles. In contrast, the score-based KSD flow does not require samples of $\pi$, and successfully converges. This suggests that the geometrical properties of the KSD flow are more favorable than the ones of the regular MMD flow. In other words, choosing an appropriate (target-dependent) kernel, as in our method or in LAWGD, appears more propitious than simply taking a general kernel $k$ unrelated to $\pi$.%\ak{maybe we should hypothesize that score based is better than sample based? :p}\pca{It's clear it is the case, you know much more from the score than from a few samples. But sometimes there is no score for $\pi$}



==> KSD descent/theory.tex <==


\section{Theoretical properties of the KSD flow}\label{sec:convergence}

In this section, we provide a theoretical study of the convergence of the KSD Wasserstein gradient flow, assessing the convexity of $\cF$ and discussing the stationary points of its gradient flow. Remarkably, we encounter pitfalls similar to other deterministic flows derived from IPMs. This issue arises because IPMs are always mixture convex, but seldom geodesically convex. We first investigate the convexity properties of $\cF$ along $W_2$ geodesics and show that exponential convergence near equilibrium cannot hold in general. Then, we examine some stationary points of its $W_2$ gradient flow, which explain the failure cases met in \Cref{sec:experiments}, where $\hat{\mu}_n$ converges to a degenerate measure.

%\ak{we provide a detailed analysis under 2 classical viewpoints: convexity or stationary points of the lyapunv. Remarkbly we encounter the same pitfalls as other deterministic flows derived from IPMS. (which give deterministic flows and do not have good W2 convexity properties) }

\subsection{Convexity properties of the KSD flow}

As is well-known, decay along $W_2$ gradient flows can be obtained from convexity properties along geodesics. A natural object of interest is then the Hessian of the objective $\cF$. We define below this object, in a similar way as \citet{duncan2019geometry}. We recall that  $\{\nabla \psi,\enspace \psi\in C_c^{\infty}(\X)\}$ is by definition dense in $\mathcal{T}_{\mu}\cP_2(\R^d)\subset L^2(\mu)$ for any $\mu\in \cP_2(\X)$ \citep[Definition 8.4.1]{ambrosio2008gradient}.% In this section, we assume that $s\in C^2(\R^d)$ so that the Hessian of $\kpi$ is well defined.
\begin{definition}\label{def_Hessian}
Consider $\psi\in C_c^{\infty}(\X)$ and the path $\rho_t$ from  $\mu$ to $(I+\nabla\psi)_{\#}\mu$ given by: $\rho_t=  (I+t\nabla\psi)_{\#}\mu$, for all $t\in [0,1]$.
The Hessian of $\cF$ at $\mu$, $H\cF_{|\mu}$, is defined as a symmetric bilinear form on $C_c^{\infty}(\X)$ associated with the quadratic form
$\Hess_{\mu}\cF(\psi,\psi) := \frac{d^2}{dt^2}\Bigr|_{\substack{t=0}}\mathcal{F}(\rho_t).$
%\begin{equation*}
%    \Hess_{\mu}\cF(\psi,\psi) := \frac{d^2}{dt^2}\Bigr|_{\substack{t=0}}\mathcal{F}(\rho_t).
%\end{equation*}
\end{definition}
\Cref{def_Hessian} can be straightforwardly related to the usual symmetric bilinear form defined on $\mathcal{T}_{\mu}\cP_2(\R^d)\times \mathcal{T}_{\mu}\cP_2(\R^d)$ \citep[Section 3]{otto2000generalization}\footnote{The $W_2$ Hessian of $\cF$, denoted $H\cF_{|\mu}$ is an operator over $\mathcal{T}_{\mu}\mathcal{P}_2(\X)$ verifying $\ps{H\cF_{|\mu}v_t, v_t}_{L^2(\mu)}=\frac{d^2}{dt^2}\Bigr|_{\substack{t=0}}\mathcal{F}(\rho_t)$ if $t\mapsto \rho_t$ is a geodesic starting at $\mu$ with vector field $t\mapsto v_t$.}.
%Our definition resembles the one of \citet{duncan2019geometry} and slightly differs from the definition the $W_2$ Hessian of $\cF$ one can encounter in the literature on Wasserstein gradient flows, see for instance \citep[Section 3]{otto2000generalization}. The $W_2$ Hessian of $\cF$, denoted $Hess\cF_{|\mu}$ is an operator over verifying $\ps{Hess\cF_{|\mu}V_t, V_t}_{L^2(\mu)}=\frac{d^2}{dt^2}\Bigr|_{\substack{t=0}}\mathcal{F}(\rho_t)$ if $t\mapsto \rho_t$ is a geodesic starting at $\mu$ with vector field $t\mapsto V_t$.\ak{added this}
\begin{proposition}\label{prop:hessian_ksd_mu}
Under \Cref{ass:lipschitz,ass:square_der_int}, 
the Hessian of $\cF$ at $\mu$ is given, for any $\psi \in C_c^{\infty}(\R^d)$, by
\begin{multline}\label{eq:hessian_ksd_mu}
\hspace{-0.4cm}   \Hess_{\mu}\cF(\psi,\psi) = \E_{x,y\sim \mu}\left[\nabla\psi(x)^T\nabla_{1}\nabla_2 \kpi(x,y)\nabla\psi(y) \right] \\
    + \E_{x,y\sim \mu}\left[\nabla\psi(x)^T H_{1}\kpi(x,y)\nabla\psi(x) \right].
    %\iint \nabla\psi(x)^T\nabla_{1,2} \kpi(x,y)\nabla\psi(y)d\pi(x)d\pi(y)
\end{multline}
\end{proposition}\vspace{-3mm}
A proof of \Cref{prop:hessian_ksd_mu} is provided in \Cref{sec:proof_hessian_ksd_mu}. Our computations are similar to the ones in \citep[Lemma 23]{arbel2019maximum} with some terms getting simpler owing to the Stein's identity satisfied by the Stein kernel. As for the squared MMD \citep[Proposition 5]{arbel2019maximum}, the squared KSD is unlikely to be geodesically convex. Indeed, while the first term is always positive, the second term in \eqref{eq:hessian_ksd_mu} can in general take negative values, unless $H_1 \kpi(x,y)$ is positive for all $x,y\in \supp(\mu)$. %A notable exception is the case of a Gaussian target $\pi\propto \exp(-x^2/2\sigma^2)$ and a linear kernel $k(x,y)=xy$, where $H_1 \kpi(x,y)=2y^2/\sigma^2\ge 0$. 
Nevertheless, at $\mu=\pi$, this second term vanishes, again owing to the Stein's property of $\kpi$.% This guarantees the local convexity of $\cF$ on a neighborhood of $\pi$ in $(\cP_2(\X),W_2)$.%an integrability assumption on $H_1 \kpi$


\begin{corollary}\label{prop:hessian_ksd_pi}
Under \Cref{ass:lipschitz,ass:square_der_int,ass:integrable}, the Hessian of $\cF$ at $\pi$ is given, for any $\psi \in C_c^{\infty}(\R^d)$, by
\begin{equation*}
    \Hess_{\pi}\cF(\psi,\psi) = \| S_{\pi,\kpi}\cL_{\pi} \psi\|^2_{\Hkpi}
    %\E_{x,y\sim \pi}\left[\nabla\psi(x)^T\nabla_{1}\nabla_2 \kpi(x,y)\nabla\psi(y) \right],
    %\iint \nabla\psi(x)^T\nabla_{1,2} \kpi(x,y)\nabla\psi(y)d\pi(x)d\pi(y)
\end{equation*}
where $S_{\pi,\kpi}$ and $\cL_{\pi}$ are defined in \Cref{eq:integral_operator,eq:def_diffusion_op}.
\end{corollary}
%, boiling down to successive integration by parts,
A proof of \Cref{prop:hessian_ksd_pi} is provided in \Cref{sec:proof_hessian_ksd_pi}. We now study the curvature properties near equilibrium, characterized by $\Hess_{\pi}\cF$. In particular, inspired by the methodology described in \citet{villani2003optimal} and recently applied by \citet{duncan2019geometry}, we expect exponential convergence of solutions initialized near $\pi$ whenever the Hessian is bounded from below by a quadratic form on the tangent space of $\cP_2(\X)$ at $\pi$, included in $L^2(\pi)$.
%denoted $\mathcal{T}_{\pi}\cP_2(\X)$, which is a subset of $L^2(\pi)$. 
\begin{definition}\label{def:exp_decay}
We say that \textit{exponential decay near equilibrium} holds if there exists $\lambda>0$ such that for any $\psi \in C_c^{\infty}(\R^d)$,
\begin{equation}\label{eq:exp_decay}
\Hess_{\pi}\cF(\psi,\psi) \ge \lambda  \|\nabla \psi\|^2_{L^2(\pi)}.
\end{equation}
%holds for any $\psi \in C_c^{\infty}(\R^d)$.
\end{definition}\vspace{-3mm}
%In other words, we expect an exponential decay of the gradient flow near the optimum, if the Hessian is a strictly positive definite quadratic form on the tangent space at $\pi$. From \Cref{prop:hessian_ksd_pi} we can see that \Cref{def:exp_decay} will hold if and only if \pca{$\psi$ rather? Is it useful?}
%\begin{equation} \label{eq:poincare_dual_form}
%    \| S_{\pi,\kpi}\cL_{\pi} \psi\|^2_{\Hkpi} \geq \lambda_{\pi} \Vert \nabla \psi \Vert_{L_2(\pi)}^2,
%\end{equation}
According to \Cref{prop:hessian_ksd_pi}, \eqref{eq:exp_decay} can be seen as a kernelized version of the following form of the Poincaré inequality for $\pi$ \citep[Chapter 5]{bakry2013analysis}
\begin{equation} \label{eq:poincare_dual_form}
    \Vert \cL_{\pi} \psi \Vert_{L_2(\pi)}^2 \geq \lambda_{\pi} \Vert \nabla \psi \Vert_{L_2(\pi)}^2.
\end{equation}
Condition \eqref{eq:exp_decay} is similar to the Stein-Poincaré inequality \citep[Lemma 32]{duncan2019geometry}. We will now argue that \eqref{eq:exp_decay} is hardly ever satisfied, thus obtaining an impossibility result reminiscent of the one for SVGD in \citep[Lemma 36]{duncan2019geometry}, which states that exponential convergence (of the KL) for the SVGD gradient flow does not hold whenever $\pi$ has exponential tails and the derivatives of $\nabla \log \pi$ and $k$ grow at most at a polynomial rate. We start with the following characterization of exponential decay near equilibrium:%We note that our proof technique and result are significantly different. 
%The above condition can be understood as a linearization of the Polyak-Lukasiewicz (PL) inequality for KSD flow around $\pi$. In other words, we expect the PL-inequality to hold locally on a neighbourhood of $\pi$, if and only if its linearization holds pointwise at $\pi$. For the KL-divergence, the role of PL-inequality is played by the log-Sobolev inequality, whose linearization around $\pi$ is the Poincaré inequality \cite{villani2003optimal}:
%\begin{equation*}
%    \Vert \nabla \psi \Vert_{L_2(\pi)}^2 \geq \lambda_{\pi} \Vert \psi \Vert_{L_2(\pi)}^2
%\end{equation*}
%for all Lipschitz $\psi$ with $\int \psi d\pi = 0$. Using the spectral decomposition of $\cL_{\pi}$, the above inequality can be easily seen to be equivalent to
%\begin{equation} \label{eq:poincare_dual_form}
%    \Vert \cL_{\pi} \psi \Vert_{L_2(\pi)}^2 \geq \lambda_{\pi} \Vert \nabla \psi \Vert_{L_2(\pi)}^2.
%\end{equation}
%To ilustrate this point, we bring to attention a more familiar example of KL-divergence. Note that the PL-inequality for KL-divergence is the log-Sobolev inequality (...), whose
%\Cref{def:exp_decay} is motivated by an analogy to how the Poincaré inequality characterizes the local exponential decay of KL-divergence for the KL-gradient flow. This follows from the fact, that the Poincaré inequality is a linearization around $\pi$ of the log-Sobolev inequality. 
%\citep[Theorem 4.4]{pavliotis2014stochastic}. 

%KSD exponential decay near equilibrium hence differs by involving the kernel integral operator $S_{\pi,\kpi}$.

%\begin{remark}\label{def:poincare}
%Recall that $\pi$ satisfies a \textit{Poincaré inequality} with constant $\lambda_{\pi}$, if
%\begin{equation}\label{eq:poincare}
   %\E_{\pi}[\| \nabla f\|] 
%  \|\mathcal{L}\psi\|^2_{L^2(\pi)}
%  \ge \lambda_{\pi} \| \nabla \psi\|^2_{L^2(\pi)}
%  %Var_{\pi}(\psi)
%\end{equation}
%for all locally Lipschitz functions $f\in L^2(\psi).$ \ak{@Szymon can the r.h.s. be written as $\|\nabla \psi\|$? se my computations in Appendix.}
%\end{remark}


%From \Cref{prop:hessian_ksd_pi} and \Cref{def:exp_decay}, we can see that the curvature properties near equilibrium will depend on whether a kernelized version of Poincare inequality \eqref{eq:poincare_dual_form} holds, similarly as in \citep[Lemma 32]{duncan2019geometry}. This condition is made explicit in the following proposition.
%This will of course depend on the choice of $k$ and $\pi$. 

\begin{proposition}\label{prop:no_exp_cv}  Let $T_{\pi,\kpi}=S_{\pi,\kpi}^* \circ S_{\pi,\kpi}$ and $L_0^2(\pi)=\{\phi \in L^2(\pi), \int \phi d\pi = 0\}$. The exponential decay near equilibrium \eqref{eq:exp_decay} holds if and only if $\cL_{\pi}^{-1} : L_0^2(\pi) \rightarrow L_0^2(\pi)$, the inverse of $\cL_{\pi}\vert_{L_0^2(\pi)}$, is well-defined, bounded, and for all $\phi \in  L_0^2(\pi)$ we have
 \begin{equation}\label{eq:proof_prop_no_exp_cv_reformulation_main}
     \langle \phi , T_{\pi, \kpi} \phi \rangle_{L_2(\pi)} \geq \lambda \langle \phi , \cL_{\pi}^{-1} \phi \rangle_{L_2(\pi)}.
 \end{equation}
 \end{proposition}\vspace{-3mm}
%The above proposition under which \eqref{eq:exp_decay} holds can be made more explicit by considering the eigendecompositions of the kernel integral operator and the Langevin diffusion operator. 
See \Cref{sec:no_exp_cv} for a proof. By the spectral theorem for compact, self-adjoint operators \citep[Section 8.3]{kreyszig1978introductory}, $T_{\pi,\kpi}$ has a discrete spectrum $(l_n)_{n\in \mathbb{N}^*}$ which satisfies $l_n\ge0$ and $l_n\to 0$. Under mild assumptions on $\pi$, the operator $\cL_{\pi}$ also has a discrete, positive spectrum \citep[Appendix A]{chewi2020svgd}. \Cref{prop:no_exp_cv} implies the following necessary condition on the spectrum of $\cL_{\pi}^{-1}$ and $T_{\pi,\kpi}$ for the exponential decay near equilibrium \eqref{eq:exp_decay} to hold.
%for the exponential decay near equilibrium and the related impossibility result.

\begin{corollary} \label{coro:spectr_decay}\
%If exponential decay near equilibrium \eqref{eq:exp_decay} holds, and the RKHS for $\kpi$ is infinite dimensional, then $\cL_{\pi}^{-1}$ has a discrete spectrum.
If $\cL_{\pi}^{-1}$ has a discrete spectrum $(\lambda_n)_{n\in \mathbb{N}^*}$ and \eqref{eq:exp_decay} %the exponential decay near equilibrium 
holds, then
% \begin{equation*}
   $  \lambda_n=\mathcal{O}(l_n)$,
% \end{equation*}
 i.e.\ the eigenvalue decay of $\cL_{\pi}^{-1}$ is at least as fast as the one of $T_{\pi,\kpi}$.
\end{corollary}
% However, \Cref{coro:spectr_decay} is hardly  satisfied, even for a standard Gaussian, as stated in the following result.

We also show that if $\Hkpi$ is infinite dimensional and exponential convergence near equilibrium holds, then $\cL_{\pi}^{-1}$ has a discrete spectrum (\Cref{lem:discrete_spectrum_hkpi}). 
We now present our impossibility result on the exponential decay near equilibrium.

\begin{theorem}\label{cor:no_exp_decay}
%Assume that $\pi$ is a Gaussian distribution on $\R^d$. Then exponential decay near equilibrium \eqref{eq:exp_decay} does not hold.
Let $\pi \propto e^{-V}$. Assume that $V \in C^2(\R^d)$, $\nabla V$ is Lipschitz and $\cL_{\pi}$ has a discrete spectrum. Then exponential decay near equilibium does not hold.
\end{theorem} 
%sec:proof_eigenvalue_decay

The main idea behind the proof of \Cref{cor:no_exp_decay}  (\Cref{sec:eigenvalue_decay_proof}) is that $T_{\pi,\kpi}$ is nuclear \citep[Theorem 4.27]{steinwart2008support}, which implies that its eigenvalues $(l_n)_{n\in \mathbb{N}^*}$ are summable. On the other hand the eigenvalue decay of $\cL_{\pi}^{-1}$ when $\pi$ is a Gaussian can be seen to be of order $O(1/n^{1/d})$ (\Cref{lem:eigenvalue_decay} in \Cref{sec:eigenvalue_decay_proof}), which is not summable. The general case is obtained by comparison with a Gaussian.
%Remark that by \Cref{lem:discrete_spectrum_hkpi}, the assumption that $\cL_{\pi}$ has a discrete spectrum in \Cref{cor:no_exp_decay} can be exchanged for an assumption that $\Hkpi$ is infinite dimensional, which is discussed in the proof of \Cref{cor:no_exp_decay}.\ak{not clear because Lemma 16 assumes exponential decay}
Despite the lack of (strong) geodesic convexity near equilibrium, we still observe empirically good convergence properties of the KSD flow for discrete measures to a stationary measure. Hence, we now investigate these stationary measures.% in the next section.

 %Indeed, on the one hand $\int \kpi(x,x')d\pi(x)d\pi(x')<\infty$ implies that the eigenvalues of $T_{\pi,\kpi}$ are 2-summable, i.e. $\sum_{n\in \mathbb{N}^*}l_n^2<\infty$ \cite{steinwart2012mercer}, hence the eigenvalues of $T_{\pi,\kpi}$ decay at most at a $\mathcal{O}(1/n)$ rate. Moreover, if $\kpi$ is bounded, the eigenvalue decay of $T_{\pi,\kpi}$ is linear (independently of the reference measure $\pi$) \citep[Theorem 2]{belkin2018approximation}. 
%\Cref{cor:no_exp_decay} states an impossibility result for  exponential convergence near equilibrium for the KSD gradient flow when the target is Gaussian. Indeed, on one hand, the eigenvalue decay of $\cL_{\pi}^{-1}$ in this case is very slow, e.g. $m_n\propto 1/n$ for a standard Gaussian in $1$ dimension \cite{bakry2013analysis}. On the other hand, $T_{\pi,\kpi}$ is nuclear \citep[Theorem 4.27]{steinwart2008support}, which implies that its eigenvalues $(l_n)_{n\in \mathbb{N}^*}$ are summable and hence should converge strictly faster than $1/n$ .
%This observation shares similarities with the impossibility result  \citep[Lemma 36]{duncan2019geometry} on SVGD, which states that exponential convergence for the SVGD gradient flow does not hold whenever $\pi$ has exponential tails and the derivatives of $\nabla \log \pi$ and $k$ grow at most at a polynomial rate.
%While studying convexity properties of $\cF$ is a natural approach, the KSD flow encounters similar issues already encountered in the study of the geodesic convexity of the squared MMD \citep[Proposition 5]{arbel2019maximum} which shows that it is not geodesically convex in general. 


%\pca{Whichever gradient we choose, minimal (Cauchy-Lipschitz style) assumptions on $v_t$ to ensure existence of solutions (for all initial conditions) are that ``$v(t,y)$ is Carathéodory, i.e. $v(\cdot,y)$ measurable and $v(t,\cdot)$ continuous, and satisfies sublinear growth $|v(t,y)|\le m(t)(1+\|y\|)$ with $m(\cdot)\in L^1([0,T],\R_+)$``. For unicity you need Lipschitz regularity, ``For any compact set $K \subset \R^d,$ there exists a map $l_{K}(\cdot) \in L^{1}\left([0, T], \R_{+}\right)$ such that the Lipschitz constant satisfies $\operatorname{Lip}(v(t, \cdot) ; K) \leq l_{K}(t)$ for a.e.\ $t \in[0, T]$``. This Lipschitz part looks like the assumption you mention.}


%\pca{So if I understand well, we have three objects determining the continuous evolution of $\mu_t$: one is the continuity equation written in the measure space, one is the $W_2$ gradient in the function space, one is the Stein (Langevin) dynamic over the particles composing the measure. We deduce: from the continuity equation, a Lyapunov function, forcing the measure to converge to the largest invariant set of \eqref{eq:ksd_flow} (a.k.a.\ LaSalle principle); from the gradient, the push-forward time discretization \eqref{eq:ksd_descent}; from the Langevin-like dynamics, an update rule on the particles. One question is: how large is the invariance set? It corresponds to vanishing KSD, can it be written as $\pi+\Sp(\nu^\pi_0,\nu^\pi_1..)$? If $k$ is universal/characteristic, then one would expect that derivating it once to obtain the Stein kernel cannot generate a large orthogonal space. In other words, maybe the Stein kernel is not characteristic, but if we can characterize where it is not, then we can try to ``avoid`` this measure subspace in the evolution of the particles (Anna said that it was empirically observed that the particles converge to $\pi$+``something``). We can add the discussion on the three types of terms (free energy, entropy and interaction) and underline that including entropy generates randomness/Brownian-Gaussian noise and this is what impedes SVGD from relying on proper non-convex optimization, whereas we have deterministic vector fields.}

%\pca{After 05/01 session: It sounds like we have a working technique that achieves convergence except for a subset of $\X$ which seems to have several interpretations: places where $\nabla_x \kpi$ is colinear with $\nabla \log \pi$, central variety defining an invariant set for our dynamics, null eigenvalue of some kernel operator related to $\kpi$. In any case this set is of dimension strictly lower than the ambient space and has some geometrical stable properties (bisectors of the polygon for which the vertices are the means of the Gaussian mixture). @Anna \& Pierre would be satisfied if we could remove/investigate this phenomenon. It seems that perturbing the Stein kernel by adding more weight to the two middle components does the trick. This could be related to adding a regularizing functional to the objective.}


\subsection{Stationary measures of the KSD flow}\label{sec:spurious_minima}

The KSD gradient flow leads to a deterministic algorithm, as for SVGD and LAWGD. To study the convergence of these algorithms in continuous time, it is relevant to characterize the stationary measures, i.e.\ the ones which cancel the dissipation $\dcF$ \eqref{eq:Lyap_deriv} of the objective functional $\cF$ along the relative gradient flow dynamics. Unfortunately, unlike for the SVGD and LAWGD algorithms, the dissipation related to the KSD flow \eqref{eq:dissipation} does not yield a dissimilarity between measures. 
Consequently, the study of the stationary measures of the KSD is more involved. We discuss below when failure cases may happen.%, as for the MMD gradient flow
%However, while the latter dynamics always converge to $\pi$ under appropriate assumptions on $\dcF$ (recall that the LAWGD dissipation cancels the $\chi^2$ divergence while SVGD dissipation cancels the square KSD, see \Cref{sec:related_work}),

\begin{lemma}\label{lem:no_cst}
Assume \Cref{ass:integrable} holds. Then $\Hkpi$ does not contain non-zero constant functions.
\end{lemma}
A proof of \Cref{lem:no_cst} is provided in \Cref{sec:proof_no_cst}. This result has the immediate consequence of considerably restricting the number of candidate fully-supported measures that are stationary for the KSD gradient flow. Consider one such measure $\mu_{\infty}$. At equilibrium, $\dot{\cF}(\mu_{\infty})=0$; which implies that $\int \kpi(x,.)d\mu_{\infty}(x)$ is $\mu_{\infty}$-a.e. equal to a constant function $c$. Since $x\mapsto c$ is then also an element of $\Hkpi$, the previous lemma implies that $c=0$. Hence, if $\mu_{\infty}$ and $\pi$ are full-support, $\cF(\mu_\infty)=0$. Provided $\kpi$ is characteristic \citep{bharath2011charac}, then $\mu_{\infty}=\pi$.%\ak{misleading sentence} , which is the case for any translation-invariant kernel with non-vanishing Fourier transform \citep[][Theorem 7]{bharath2008fourier} such as the Gaussian or IMQ kernels

However, as  \Cref{alg:ksd_descent_GD,alg:ksd_descent_LBFGS} rely on discrete measures, the dissipation $\dcF$ \eqref{eq:dissipation} can vanish even for $\mu\neq \pi$ because $\mu$ is not full-support. Depending on the properties of $\pi$ and $k$, this may happen even for trivial measures such as a single Dirac mass, as stated in the following Lemma.
\begin{lemma}\label{cor:stable Dirac}
Let $x_0$ such that $s(x_0)=0$ and $Js(x_0)$ is invertible, and consider a translation-invariant kernel $k(x,y)=\phi(x-y)$, for $\phi\in C^3(\X)$. Then $\delta_{x_0}$ is a stable fixed measure  of \eqref{eq:ksd_flow}, i.e. it is stationary
and any small push-forward of $\delta_{x_0}$ is attracted back by the flow.
\end{lemma}%\ak{we should explain to the reader why its not good. that it happens not only on the modes of distribution}
\emph{Proof:} For $\varepsilon > 0$ and $\psi\in C^\infty_c(\R^d)$, set $\mu_{\varepsilon} = (I + \varepsilon \psi)_\#\delta_{x_0} $. We then have $\cF(\mu_{\varepsilon}) =\frac{1}{2} \kpi(x_0 + \varepsilon \psi(x_0), x_0 + \varepsilon \psi(x_0))$.
Expanding $\kpi(x, x)$ at the first order around $x = x_0$ gives $2\cF(\mu_{\varepsilon}) = \varepsilon^2 \|[Js(x_0)]\psi(x_0)\|^2 \phi(0)-\Delta \phi(0) + o(\varepsilon^2)$.
This quantity is minimized for $\psi(x_0) = 0$, which shows that $\delta_{x_0}$ is indeed a local minimum for $\cF$.
%\ak{measurable map? L2 map?}\pca{$C^\infty_c$ would be enough?}\pab{Isn't it just continuous? Since we only look as phi(x0), it does not matter much}

Importantly, this result applies whenever the score $s$ vanishes at $x_0$, not only when $x_0$ is a local stable minimum of the potential $\log(\pi)$. This means that for a single particle, KSD descent is attracted to any stationary point of $\log(\pi)$, whereas SVGD converges only to local maxima of $\log(\pi)$ \cite{liu2016stein}. Nonetheless, if $\pi$ is log-concave, there is no spurious stationary point.

%\begin{remark} For $\mu_0=\delta_{x_0}$ and a translation-invariant $k$, the dissipation $\dot{\mathcal{F}}(\delta_{x_0})$ vanishes if and only if $x_0$ is a stationary point of $x\mapsto\|s(x)\|^2$, i.e.\ $[Js(x_0)]s(x_0) = 0$. Therefore, if $\pi$ is log-concave (meaning that $Js$ is negative definite), and we denote by $x^*$ its maximum, the dissipation vanishes if and only if $x_0 = x^*$: the KSD flow for a single Dirac mass has no spurious stationary point for log-concave targets $\pi$.
%\end{remark}
For cases more general than \Cref{cor:stable Dirac}, we are interested in the sets that are kept invariant by the gradient flow. For these sets, an erroneous initialization may prevent the particles from reaching the support of $\pi$. We provide below a general result holding for any deterministic flow, beyond our specific choice \eqref{eq:ksd_flow} of $v_{\mu_t}$, and thus holding also for SVGD. %It involves contingent cones which are crucial quantities for studying the invariance of non-smooth sets. They can be informally described as the collection of directions at $x$ that point either inward or tangent to the set $\cM$. More formally, for $d_\cM(y)$ the distance of $y\in\X$ to $\cM$, $T_\cM(x):=\{v|\liminf\limits_{h\rightarrow 0^+} d_\cM(x+h v)/h=0\}$.

\begin{definition}
Let $\cM\subset \R^d$ be a closed nonempty set. We say that $\cM$ is a flow-invariant support set for the flow $(\mu_t)_{t\ge 0}$ of \eqref{eq:continuity_eq} if for any $\mu_0$ s.t.\ $\supp(\mu_0)\subset \cM$, we have that the flow verifies $\supp(\mu_t)\subset \cM$ for all $t\ge 0$.
\end{definition}

\begin{proposition}\label{prop:stable support}(Informal)
Let $\cM\subset \R^d$ be a smooth nonempty submanifold and $\mu_0\in \cP_c(\X)$ with $\supp(\mu_0)\subset\cM$. Assume that, for a deterministic $(v_{\mu_t})_{t\ge 0}$ satisfying classical Caratheodory-Lipschitz assumptions (\Cref{sec:Cauchy-Lip_flow}), we have $v_{\mu_t}(x)\in T_\cM(x)$ where $T_\cM(x)$ is the tangent space to $\cM$ at $x$. Then $\cM$ is flow-invariant for \eqref{eq:continuity_eq}.% is the contingent cone of $\cM$ at $x\in \cM$ Based on an invariance result from nonsmooth analysis,\pab{Should say that its in the appendix, and maybe just say that the prop in informal}
\end{proposition}
%\emph{Proof idea:} We first show that any point $x_0\in \supp(\mu_0)$ would generate a trajectory $x'(t)=v_{\mu_t}(x(t))$ which stays within $\cM$ at all times. Then the superposition principle allows to conclude for the support of the measures $\mu_t$.  
%\ref{ass:caratheodory_field_contr}-\ref{ass:lip_field_wrtMeasure_contr} 

The formal statement, \Cref{prop:stable_support_nonsmooth}, stated and proved in \Cref{sec:proof_stable_support}, can be in particular applied to the ubiquitous radial kernels and to planes of symmetry of $\pi$, i.e.\ affine subspaces $\cM\subset \R^d$ such that the density of $\pi$ is symmetric w.r.t.\ $\cM$. \Cref{lem:Flow-invariant symmetry} is illustrated in \Cref{sec:experiments} for a mixture of two Gaussians with the same variance (\Cref{fig:mog_problem}).

\begin{lemma}\label{lem:Flow-invariant symmetry}
Let $\cM$ be a plane of symmetry of $\pi$ and consider a radial kernel $k(x,y)=\phi(\|x-y\|^2/2)$ with $\phi\in C^3(\R)$. Then, for all $(x,y)\in\cM^2$, $\nabla_{2}\kpi(x,y)\in T_\cM(x)$ and $\cM$ is flow-invariant for \eqref{eq:ksd_flow}.
\end{lemma}
\emph{Proof idea:} We show that all the terms in $\nabla_{2}\kpi(x,y)$ belong to $T_\cM(x)$. This implies that the convex combination $\nabla_{W_2}\cF(\mu)(y)=\mathbb{E}_{x \sim \mu}[\nabla_{2}\kpi(x,y)]\in T_\cM(x)$. We then apply \Cref{prop:stable support} to conclude.


%\pca{Other possible results: existence of a local extremum on the subspace}

==> auxiliary_results.tex <==

\begin{lemma}
	Assume that $k : \R^n \times \R^n \rightarrow \R$ is a kernel, such that $k(\cdot, x)$ is $\lambda$-convex for all $x \in \R^n$. Let $H$ be the RKHS of $k$ and assume it is separable. Then the functional
	$$\mathcal{W}_k = \int_{\R^n}\int_{\R^n} k(x,y) \mu(dx) \mu(dy)$$
	is $\lambda$-geodesically convex on $(\mathcal{P}_2(\R^n), W_2)$.
\end{lemma}
\begin{proof}
	Let $\mu_0, \mu_1 \in \mathcal{P}_2(\R^n) \cap \mathcal{P}_k(\R^n)$. Since the kernel is measurable and RKHS $H$ is separable, the kernel mean embeddings:
	$$ \hat{\mu}_i = \int k(\cdot, x) \mu_i(dx) $$
	exist for $i \in \{0,1\}$. Furthermore, $\mathcal{W}_k(\mu_i) = \Vert \hat{\mu}_i \Vert_H^2$ for $i \in \{0,1\}$. 
	
	Let $\pi \in \Pi(\mu, \nu)$ be an optimal transport plan between $\mu_0$ and $\mu_1$ and let $0 < t < 1$. We have:
	\begin{align*}
	\mathcal{W}_k(\mu_t) = & \iint k((1-t) x_1 + tx_2 , (1-t) y_1 + ty_2)  \pi(dx_1, dx_2) \pi(dy_1, dy_2)  \\ 
	&\leq  \iint (1-t) k(x_1, (1-t)y_1 + t y_2) + t k(x_2, (1-t)y_1 + ty_2) - t(1-t)\frac{\lambda}{2} \Vert x_1 - x_2 \Vert_2^2 \pi(dx_1, dx_2) \pi(dy_1, dy_2)  \\
	& \leq \iint (1-t)^2 k(x_1, y_1) + t(1-t) (k(x_1, y_2) + k(x_2, y_1)) + t^2 k(x_2, y_2) \pi(dx_1, dx_2) \pi(dy_1, dy_2) \\
	& \hspace{10pt} - \iint t(1-t)\frac{\lambda}{2} (\Vert x_1 -x_2 \Vert_2^2 + \Vert y_1 - y_2 \Vert_2^2) \pi(dx_1, dx_2) \pi(dy_1, dy_2) \\
	& = \Vert (1-t) \hat{\mu}_0 +  t\hat{\mu}_1 \Vert_H^2 - t(1-t)\lambda W_2^2(\mu_0, \mu_1) \\
	& = (1-t) \mathcal{W}_k(\mu_0) + t \mathcal{W}_k(\mu_1) - t(1-t) \Vert \hat{\mu}_0 - \hat{\mu}_1 \Vert_H^2 - \lambda t(1-t) W_2^2(\mu_0, \mu_1) \\
	& \leq  (1-t) \mathcal{W}_k(\mu_0) + t \mathcal{W}_k(\mu_1) - \lambda t(1-t) W_2^2(\mu_0, \mu_1)
	\end{align*}
	which proves the thesis.
	
	
	\begin{lemma}{Distance to constant functions}
		
		Let $f: \R^p \to \R$ such that for all $x$, the mapping $y\mapsto k_{\pi}(x, y) f(y)$ is integrable and call $\phi(x) = \int_{y} k_{\pi}(x, y) f(y) dy - 1$.
		Using Fubini, we find:
		$\int_{x} \phi(x) \pi(x)dx = -1$.
		Then, for a target measure $\mu$ such that $\pi / \mu$ is defined everywhere, it holds
		\begin{align*}
		1 &= \left\lvert\int_{x} \phi(x) \pi(x)dx\right\lvert\\
		&= \left\lvert\int_{x} \phi(x) \sqrt{\mu(x)} \frac{\pi(x)}{\sqrt{\mu(x)}}dx\right\lvert\\
		&\leq \left(\int_x \phi^2(x)d\mu(x)\right)\times \left(\int_{x}\frac{d\pi}{d\mu}(x) d\pi(x)\right)
		\end{align*}
		Which gives the bound
		$$
		\|\phi\|_{L^2(\mu)} \geq \left(\int_{x}\frac{d\pi}{d\mu}(x) d\pi(x)\right)^{-1}
		$$
	\end{lemma}
\end{proof}

\begin{lemma}{Analysis of stationary points}
	
	Consider a $2$d case, and a density $\pi$ symmetric w.r.t. the $y$ axis, i.e. $\pi(x, y) = \pi(-x, y)$. We call $\mathcal{M}$ the axis.
	
	We call $\tilde{\pi}$ the density $\R \to \R$ such that $\tilde{\pi}(0, y) \propto \pi(0, x)$.
	%
	
	Let $\mu : \R^2\to \R$ a density such that $\supp(\mu)\subset \mathcal{M}$.
	%
	We call $\tilde{\mu}$ the projection of $\mu$ on $\mathcal{M}$.
	We assume that $k$ is written as $k(x, y) = \phi(\|x - y\|^2)$, with $\phi$ decreasing.
	
	We find:
	
	$$
	KSD^2(\mu, \pi) = KSD^2(\tilde{\mu},\tilde{\pi}) - \int_{\mathcal{M}^2} \phi'(\|x -y\|)^2 d\tilde{\mu}(x)d\tilde{\mu}(y)
	$$
	
	Let $\tilde{\mu} = (I + \psi)_{\#}\tilde{\pi}$.
	%
	A Taylor development gives:
	
	$$
	KSD^2(\mu, \pi) =-\int_{\mathcal{M}^2} \phi'(\|x -y\|)^2 d\tilde{\pi}(x)d\tilde{\pi}(y) 
	-\int_{\mathcal{M}^2} \phi"(\|x -y\|)^2\langle x - y, \psi(x) - \psi(y)\rangle d\tilde{\pi}(x)d\tilde{\pi}(y)  
	+\frac12\mathrm{Hess}_{\tilde{\pi}}(\psi, \psi)
	$$
\end{lemma}

